What do Speech Foundation Models Learn? Analysis and Applications

Speech foundation models (SFMs) are designed to serve as general-purpose representations for a wide range of speech-processing tasks. The last five years have seen an influx of increasingly successful self-supervised and supervised pre-trained models with impressive performance on various downstream tasks. Although the zoo of SFMs continues to grow, our understanding of the knowledge they acquire lags behind. This thesis presents a lightweight analysis framework using statistical tools and training-free tasks to investigate the acoustic and linguistic knowledge encoded in SFM layers. We conduct a comparative study across multiple SFMs and statistical tools. Our study also shows that the analytical insights have concrete implications for downstream task performance. The effectiveness of an SFM is ultimately determined by its performance on speech applications. Yet it remains unclear whether the benefits extend to spoken language understanding (SLU) tasks that require a deeper understanding than widely studied ones, such as speech recognition. The limited exploration of SLU is primarily due to a lack of relevant datasets. To alleviate that, this thesis contributes tasks, specifically spoken named entity recognition (NER) and named entity localization (NEL), to the Spoken Language Understanding Evaluation benchmark. We develop SFM-based approaches for NER and NEL, and find that end-to-end (E2E) models leveraging SFMs can surpass traditional cascaded (speech recognition followed by a text model) approaches. Further, we evaluate E2E SLU models across SFMs and adaptation strategies to assess the impact on task performance. Collectively, this thesis tackles previously unanswered questions about SFMs, providing tools and datasets to further our understanding and to enable the community to make informed design choices for future model development and adoption.

==> figures-tex/analysis/agwe.tex <==
\begin{figure}[btp]
    \centering
    \includegraphics[width=0.7\linewidth]{images/agwe_illustration_no_bg.png}
    \caption{Word pronunciation vectors; acoustically grounded word embeddings (AGWEs) $g(v)$ and $g(v^-)$ above are learned with speech/text multi-view training~\cite{he2017multiview}.}
    \label{fig:agwe}
\end{figure}

==> figures-tex/analysis/res-cca-linguistic.tex <==
\begin{figure*}[btp]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=0.95\linewidth, trim=0 318 0 0, clip]{images/legend-cca.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/cca_cd_agwe.pdf}
         \caption{Word pronunciation content; CCA similarity between \sfm \ word segment representations and AGWEs.}
         \label{fig:res-agwe}
     \end{subfigure}
 
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/cca_cd_syntactic.pdf}
         % \includegraphics[width=\linewidth, trim=0 130 0 75, clip]{images/cca_cd_syntactic_small.pdf}
         \caption{Syntactic content; CCA similarity between \sfm \ word segment representations and POS attributes.}
         \label{fig:res-ptb}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/cca_cd_semantic.pdf}
         \caption{Semantic content; CCA similarity between \sfm \ word segment representations and SemCor attributes.}
         \label{fig:res-semcor}
     \end{subfigure}
%  \ifdraft    
%      \begin{subfigure}[b]{\linewidth}
%          \centering
%          \includegraphics[width=\linewidth, trim=0 225 0 0, clip]{images/cca_cd_glove.pdf}
%          \caption{Semantic content as measured by CCA similarity between \sfm \ word segment representations and GloVe.}
%          \label{fig:gloveB}
%      \end{subfigure}
% \fi        
\end{minipage}
\caption{Measure of different linguistic properties using CCA for \baseM \ (left) and \largeM \ (right) \sfms.}
\label{fig:res-cca-linguistic}
\end{figure*}

==> figures-tex/analysis/res-cca-local.tex <==
\begin{figure*}[btp]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=0.95\linewidth, trim=0 310 0 0, clip]{images/legend-phone.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering     
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/intra.pdf}
         \caption{CCA similarity between \sfm \ frame-level representations and local features.}
         \label{fig:res-cca-intra}
     \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/mel.pdf}
         \caption{Spectral content; CCA similarity between \sfm \ frame-level representations and FBank features.}
         \label{fig:res-cca-mel}
     \end{subfigure}
\end{minipage}
\caption{CCA analysis for local features for \baseM \ (left) and \largeM \ (right) \sfms.}
\label{fig:res-cca-local}
\end{figure*}

==> figures-tex/analysis/res-cca-surface.tex <==
\begin{figure*}[btp]
\begin{minipage}[b]{1.0\linewidth}
\small

 \centering
 \centerline{\includegraphics[width=0.95\linewidth, trim=0 310 0 0, clip]{images/legend-word.pdf}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering     
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/phone.pdf}
         \caption{Phonetic content; CCA similarity between \sfm \ phone segment representations and phone identity.}
         \label{fig:res-cca-phone}
     \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 235 0 0, clip]{images/word.pdf}
         \caption{Word-level content; CCA similarity between \sfm \ word segment representations and word identity.}
         \label{fig:res-cca-word}
     \end{subfigure}
\end{minipage}
\caption{CCA analysis for phone and word ID encoded in span representations for \baseM \ (left) and \largeM \ (right) \sfms.}
\label{fig:res-cca-surface}
\end{figure*}

==> figures-tex/analysis/res-hubertb-metric.tex <==
\begin{figure*}[btp]
% \begin{minipage}[b]{1.0\linewidth}
% \small

 % \centering
 % \centerline{\includegraphics[width=0.95\linewidth, trim=0 318 0 0, clip]{images/legend-cca.pdf}}
% \end{minipage}
\begin{minipage}[b]{1.0\linewidth}

\centering   
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_cca_word.pdf}
         % \caption{Vanilla CCA with varying number of directions used for similarity calculation.}
         \label{fig:v-cca-hubert}
     \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_svcca_word.pdf}
         % \caption{SVCCA with varying number of directions restored based on the explained variance.}
         \label{fig:svcca-hubert}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_pwcca_cka_op_word.pdf}
         % \caption{PWCCA}
         \label{fig:pwcca-cka-op-hubert}
     \end{subfigure}

     % \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_cka_word.pdf}
     %     % \caption{Semantic content; CCA similarity between \sfm \ word segment representations and SemCor attributes.}
     %     \label{fig:cka-hubert}
     % \end{subfigure}

     %  \begin{subfigure}[b]{\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_op_word.pdf}
     %     % \caption{Semantic content; CCA similarity between \sfm \ word segment representations and SemCor attributes.}
     %     \label{fig:op-hubert}
     % \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/hubert_small_mi_word.pdf}
         \label{fig:mi-hubert}
     \end{subfigure}
\end{minipage}
\caption{Different tools comparing \sfm \ representations with word identity for \hubert-\baseM.}
\label{fig:res-hubertb-metric}
\end{figure*}

==> figures-tex/analysis/res-w2v2b-metric.tex <==
\begin{figure*}[btp]

\begin{minipage}[b]{1.0\linewidth}

\centering   
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/wav2vec_small_cca_word.pdf}
         \label{fig:v-cca-hubert}
     \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/wav2vec_small_svcca_word.pdf}
         \label{fig:svcca-hubert}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/wav2vec_small_pwcca_cka_op_word.pdf}
         \label{fig:pwcca-cka-op-hubert}
     \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth, trim=0 230 0 0, clip]{images/wav2vec_small_mi_word.pdf}
         \label{fig:mi-hubert}
     \end{subfigure}
\end{minipage}
\caption{Different tools comparing \sfm \ representations with word identity for \wavtovec-\baseM.}
\label{fig:res-w2v2b-metric}
\end{figure*}

==> figures-tex/corr-scores.tex <==
% \begin{figure}[t]
% \centering
% \begin{minipage}{.48\textwidth}
%   % \centering
% % \begin{figure}[htb]
% \footnotesize
%  \centering
%  % \centerline{\includegraphics[width=\linewidth]{images/corr_scores.pdf}}
%  \centerline{\includegraphics[width=\linewidth, trim=0 305 0 10, clip]{images/semantic_scores_1.pdf}}
%  \centerline{\includegraphics[width=\linewidth]{images/all_tasks.pdf}}
% \caption{\it Task performance and best layer for all tasks.}
% % Correlation between layer-wise CCA scores and task performance. ASR and PR performances are typically reported as error rates; we use ($100-\text{error rate}$) here for consistency, so a higher correlation is better. Scores $<0.5$ are not visible here. }
%   \label{fig:corr-scores}
% % \end{figure}
% \end{minipage}%
% \hfill
% \begin{minipage}{.48\textwidth}
%   \centering
% % \begin{figure}[t]
% \footnotesize
%  \centering
%  % \centerline{\includegraphics[width=9cm, trim=0 175 0 0, clip]{images/scatter_for_paper.pdf}}
%  \centerline{\includegraphics[width=\linewidth]{images/scatter_for_paper.pdf}}
% \caption{\it Scatter plots for specific model, task, and CCA measure combinations. Each point is labeled with its layer index.}
%   \label{fig:scatter}
% \end{minipage}%
% \end{figure}

\begin{figure}[ht]
  \begin{minipage}[c]{0.65\textwidth}
    \includegraphics[width=0.9\textwidth]{images/scatter_for_paper.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.35\textwidth}
    \caption{\it Scatter plots for specific model, task, and CCA measure combinations. Each point is labeled with its layer index
}
  \label{fig:scatter}
  \end{minipage}
\end{figure}

==> figures-tex/method-ext-ner-data.tex <==
\begin{figure}[h]
  \centering
    \includegraphics[width=0.8\textwidth]{images/method-ner-ext-data.png}
    \caption{\it Overview of how we use the external data with our baseline NER models to generate pseudo-labeled data for task-specific supervised training.
}
  \label{fig:method-ner-ext-data}
\end{figure}

==> figures-tex/metric_analysis/metric-correlation-data2vecl.tex <==
\begin{figure}[ht]
\centering

\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_phone_spearman.pdf}
    % \caption{First Image}
    \label{fig:data2vecl-phone-spearman}
\end{subfigure}
\hfill % add horizontal space
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_phone_pearson.pdf}
    \label{fig:data2vecl-phone-pearson}
    % \caption{Second Image}
\end{subfigure}


\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_word_spearman.pdf}
    % \caption{Third Image}
    \label{fig:data2vecl-word-spearman}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_word_pearson.pdf}
    % \caption{Fourth Image}
    \label{fig:data2vecl-word-pearson}
\end{subfigure}


\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_cd_semantic_50inst_spearman.pdf}
    % \caption{Third Image}
    \label{fig:data2vecl-sem-spearman}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=0 0 30 0, clip]{images/metric_analysis/data2vec_large_cd_semantic_50inst_pearson.pdf}
    % \caption{Fourth Image}
    \label{fig:data2vecl-sem-pearson}
\end{subfigure}

\caption{Four Images in a 2x2 Grid}
\label{fig:2x2grid}
\end{figure}

==> figures-tex/metric_analysis/task-pr-asr-all.tex <==
\begin{figure*}[btp]

\begin{minipage}[b]{1.0\linewidth}

\centering   
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{images/metric_analysis/scatter_plots/scatter_metrics_all_phone.pdf}
         \label{fig:pr-all}
     \end{subfigure}

     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{images/metric_analysis/scatter_plots/scatter_metrics_all_asr.pdf}
         \label{fig:asr-all}
     \end{subfigure}
    
\end{minipage}
\caption{Scatter plots comparing task-performance with task-agnostic layer-wise trends.}
\label{fig:task-pr-asr-all}
\end{figure*}

==> figures-tex/nel-dev-wer-f1.tex <==
\begin{figure}[h]
  \begin{minipage}[c]{0.65\textwidth}
    \includegraphics[width=0.95\textwidth]{images/nel_dev_wer_f1.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.35\textwidth}
    \caption{\it Example inference for an E2E NEL model using a CTC recognizer. The transcript is ``the eu funds''. `\#' and `]' are the start and end labels of an ORG entity.
}
  \label{fig:nel-dev-wer-f1}
  \end{minipage}
\end{figure}

==> figures-tex/res-ner-ext-data.tex <==
\begin{figure}[htbp]
  \begin{minipage}[c]{0.65\textwidth}
    \includegraphics[width=0.95\textwidth]{images/fscore-test.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.35\textwidth}
    \caption{\it Improvements in spoken NER E2E and pipeline approaches with 100 hours of external data -- unlabeled speech or unlabeled text or transcribed speech.
}
  \label{fig:res-ner-ext-data}
  \end{minipage}
\end{figure}

==> figures-tex/res-wordsim.tex <==
\begin{figure}[h]
  \begin{minipage}[c]{0.75\textwidth}
    \includegraphics[width=0.9\textwidth]{images/wordsim-label.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.25\textwidth}
    \caption{\it Word similarity performance (mean across tasks).
}
  \label{fig:tsne-pos}
  \end{minipage}
\end{figure}

==> sections/old_versions/analysis-old.tex <==
\newpage
\tbd{Merge from \href{https://www.overleaf.com/project/646a3dc5ea6e8b7c652d2fa3}{LRS final project}}
\section{What do the self-supervised speech models know?}
\label{sec:study}
Self-supervised speech representation models have been around for more than a decade~\cite{mohamed2022self}, with recent successes on account of smartly designed pairs of pretext task and training objective, and transformer architecture~\cite{vaswani2017attention}, a more efficient counterpart to the traditional recurrent neural networks. \tbd{More background, add figures?} The 
broad applicability and 
growing adoption of self-supervised speech representations~\cite{mohamed2022self} intensifies the need to develop a better understanding of these models.  

\tbd{A para on related work}

\subsection{Analysis Tools}
{\bf Canonical Correlation Analysis.} CCA~\cite{harold1936relations} is a statistical technique that measures the relationship between two continuous-valued random vectors as represented by the maximum correlations between their linear projections. CCA has been previously used as a measure of similarity to compare representations within and across neural network models~\cite{raghu2017svcca, kornblith2019similarity, voita2019bottom}. Here we use it in the same way, and also to measure the similarity between a layer representation and another vector, such as word embeddings or acoustic features.

CCA takes $n$ pairs of vectors $\{(x_1, y_1), ..., (x_n, y_n)\}$, sampled from the random vectors (or ``views") $X\in\mathbb{R}^{d_1}, Y\in\mathbb{R}^{d_2}$, as input and returns a correlation score as a measure of similarity between the two views.
%``views" $X$ and $Y$. 
The solution can be defined iteratively as follows: First, we define the directions of maximum correlation between linear projections of $X$ and $Y$: 
$v_1, w_1 = \argmax{v, w} \text{corr}(v^TX, w^TY)$. 
The subsequent directions $v_i, w_i \; \forall i \in [2, k]$, $k = \min(d_1, d_2)$, maximize the same correlation subject to each new projection being uncorrelated with others in the same view.

In standard CCA the {\emph canonical correlation} $\textrm{CCA}(X, Y)$ is the sum (or mean) of the correlations $\rho_i = \text{corr}(v_i^TX, w_i^TY)$. We use a variant, {\it projection-weighted CCA (PWCCA)}~\cite{morcos2018insights}, which computes a weighted mean of the $\rho_i$s, with higher weights for directions accounting for a higher proportion of the input. PWCCA has been found to be more robust to spurious correlations in the data. Since PWCCA is asymmetric, we report the mean of the two quantities $\textrm{CCA}(X, Y)$ and $\textrm{CCA}(Y, X)$. Henceforth we refer to this average as the ``CCA similarity", and it has a maximum value of 1.

As illustrated in \fig~\ref{fig:model}, we use PWCCA to measure similarity between the W2V2 layer representations and various continuous-valued quantities of interest, either (i) from a different layer of the same model ({\it CCA-intra}), (ii) from a fine-tuned version of the model ({\it CCA-inter}), or (iii) from an external representation. For the third type of analysis we use mel filter bank features ({\it CCA-mel}), acoustically grounded word embeddings~\cite{settle2019acoustically} ({\it cca-agwe})\footnote{AGWEs are trained to be close to acoustic embeddings of the corresponding words, so we expect they encode mainly acoustic-phonetics.} and GloVe word embeddings~\cite{pennington2014glove} ({\it cca-glove}) as ways to assess the local acoustic, word-level acoustic-phonetic, and word meaning information encoded in the W2V2 representations respectively.

{\bf Spoken STS}


{\bf wordsim}


{\bf Syntactic and semantic vectors}


{\bf Experimentation details}


Figure~\ref{fig:schematic} shows a high-level schematic of a present-day representation model and the different scales of information that we extract from it for our analysis experiments~\cite{pasad2021layer}. Either raw audio or filter-bank features are used as input; raw input is typically processed through a set of convolution sub-network to reduce the resolution. 
\noindent 
% In our quest to understand the strengths of the pre-trained speech representation models
To that end, in my ASRU 2021 work~\cite{pasad2021layer},
my collaborators and I
adopted lightweight probing tools -- based on canonical correlation analysis (CCA), mutual information (MI), and simple similarity tasks --  to measure the acoustic and linguistic properties encoded by
% intermediate representations of
pre-trained speech models. These tools have an edge over widely used probing classifier approaches~\cite{belinkov2019analysis}, as they avoid the overhead and
confounding effects of
% unclear dependence on 
design decisions involved in training classifiers. 
Figure~\ref{fig:trends} gives a glimpse of our findings showing where different levels of information reside in two commonly used models wav2vec2.0 small and large~\cite{baevski2020wav2vec}.

\begin{figure}[h]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  % \includegraphics[width=.9\linewidth]{images/all-in-one.png}
  \includegraphics[width=.9\linewidth]{images/all-in-one.pdf}
  \caption{\small{\it Illustration of property content~\cite{pasad2021layer}. The different metrics, not directly comparable, are shown together only to compare where major peaks and valleys occur.}}
  \label{fig:trends}
\end{minipage}%
\hfill
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=.85\linewidth]{images/model.pdf}
  % \includegraphics[width=.85\linewidth]{images/schematic.pdf}
  \caption{\small{\it Model architecture schematic when input is a raw waveform with an example showing representations extracted for different spans.}}
  \label{fig:schematic}
\end{minipage}%
\end{figure}


% The model is trained with contrastive predictive coding of the masked spans and using output of CNN module 
% The models are typically trained with pretext tasks designed using masking. 
% \tbd{Need to mention librispeech somewhere?}
Figure~\ref{fig:schematic} shows a schematic of the model and the different spans of representation that we extract for our experiments. 
We found that the features from the convolutional sub-network are highly similar to the widely used filter-bank features. This finding suggests a less computationally intensive approach that uses filter-bank features in place of the convolutional module, which has since been found by others to be a reasonable modification~\cite{wu2022performance}.
% thus suggesting a less computationally intensive approach that takes the filter-bank features as input bypassing the convolutional module. 
% Experiments done by Wu et al.~\cite{wu2022performance} show this as a reasonable modification.
% This is confirmed by Wu et al.~\cite{wu2022performance}, who implement this. 
Further, we also probed for various aspects of phonetic and word-level content. We found that all the trends follow an auto-encoder-like structure: the most high-level (contextual) information resides in the intermediate layers and the first few and last few layers are least correlated to the linguistic properties. This behavior may be attributed to the pre-training objective, which encourages the final output to be similar to the output of the convolutional module~\cite{baevski2020wav2vec}.

In more recent work with my collaborators~\cite{arxiv}, I perform a comparative study of these trends for models that differ in the input modality, training objective, and training language. For instance, when pre-training objective uses an intermediate transformer layer to define output units -- as in HuBERT~\cite{hsu2021hubert} and wavLM~\cite{chen2022wavlm} -- the auto-encoder structure is no longer present and the final few layers tend to be most contextual. 
% \tbd{not mentioning extension to other datasets}

% Our proposed approaches allow for both types of signals, discrete (labels) and continuous (external representation vectors). In \cite{pasad2021layer}, we also corroborate our findings using multiple measures, canonical correlation analysis (CCA), discrete mutual information (MI), and surface-level tasks such as word discriminability using extracted word-level representations and word similarity benchmark~\cite{faruqui2014community} using extracted context-independent word embedding map. These tools have an edge over widely used probing approaches~\cite{belinkov2019analysis}, as these avoid the overhead and unclear dependence on design decisions involved in training probing classifiers. 

\subsection{Next steps}
\label{sec:study-next-steps}
\underline{Analysis tools}: As previously discussed, I have used projection-weighted CCA~\cite{morcos2018insights}, discrete MI, and similarity tasks, in my experiments so far, but other variants of CCA~\cite{raghu2017svcca}, centered kernel alignment (CKA)~\cite{kornblith2019similarity}, and neural collapse~\cite{papyan2020prevalence} (discussed again in Sec.~\ref{sec:finetune-next-steps}) are
some
% all 
reasonable alternatives. Preliminary experiments have shown similar trends for some of these methods, but also some differences in robustness and ease of use.  My thesis work will develop a better understanding of the relative merits of different analysis tools, and produce a suite of the most successful ones for use by the research community.
% We observe similar trends from some of these tools in our previous experiments, but we would like to develop a better understanding of any similarities and differences in these measures.
% \tbd{I am not very sure of keeping this para as future work, maybe just the part that we have seen consistent trends from using these different tools (not mentioning NC).} 
%  Given pairs of representations and discrete labels, Neural collapse measures a ratio of intra-cluster variability and inter cluster variability; meaning a lower NC implies that the representations have a good separability with respect to the label set. We also use this in \cite{emnlp}, which is detailed in section~\ref{sec:emnlp}.




\sout{\underline{Analysis of contextualization}: 
The self-attention mechanism in transformer-based models enables the local representations to encode long-range speech properties, beyond the size of the input frames (typically 20ms). 
% The extraction of span representations (fig.~\ref{fig:schematic}) does not take any de-localization effects into account.
% Because of self-attention mechanism in transformer based models, the information extracted from a particular audio span may no longer be localized into the corresponding frame representation. This property also enables the self-attention layers to possibly learn long-range speech properties, possibly encoding information beyond the size of input frames (typically 20ms).
% and the quality of the representations is not constrained by the size of the input frames (typically 20ms).
% For example, self-attention in visually grounded speech models helps detect word segments~\cite{peng2022word}.
% We wish to study this contrast in the future and complement the preliminary efforts in this direction~\cite{yang2020understanding}.
I plan to study the attention structure to quantify the amount of de-localization, and furthermore how it is affected by different pre-training objectives.
% and fine-tuning. For instance, do certain downstream tasks use/learn more delocalized attention maps than others?
% , and reevaluate our previously found trends based on any delocalized self-attention structures. 
% Study of self-attention in text models using principal component analysis (PCA) found useful in previous work on text models~\cite{bhojanapalli2021eigen}.
}\tbd{make this more concrete if want to add}

\underline{Analysis of semantic content}: Our findings~\cite{pasad2021layer} indicated that the pre-trained model encoded non-trivial semantics. However, understanding the kind of semantic information encoded requires more work.  I plan to study semantic similarity tasks, such as the WordSim benchmark~\cite{faruqui2014community} and spoken sentence similarity~\cite{merkx2021semantic}.
% But we found this study incomplete in telling us what kind of semantic information is encoded by the model. So, we plan to advance this by evaluating the representations on spoken semantic textual similarity benchmark~\cite{merkx2021semantic}
% , which is a sentence similarity benchmark for dictated sentences from text STS task~\cite{textsts}. 
% Further, we plan to revisit the individual tasks that are a part of the WordSim benchmark, to abstract out any fine-grained information of encoded semantics.
Additionally, I will examine linguistic patterns present in instance-level self-attention matrices, taking inspiration from prior work studying self-attention in BERT~\cite{clark2019does}.\tbd{rethink the last part}
% similar to those previously done in text models~.  

% Inspiration from text models analysis of word contextualization? Synthetic tasks?

\subsection{Our work in context}\tbd{need to find a good placing for this}
The hierarchical structure of learned latent spaces has been seen in speech, text, and vision models before\cite{?, ?}. Probing. 
There is a lot of work analyzing text representation models using parametric probes or using synthetic tasks. Although the work does give us some valuable inspiration, the same set of techniques and experiments may not always be scalable or reasonable to speech modality because of differences such as continuous inputs, longer sequences, unsegmented input can have multiple meaningful generalities based on acoustic and linguistic aspects. Other researchers have contributed their work on analysing supervised and multi-modal approaches~\cite{1, 2}.

\subsection{Limitations}
\ap{This is work in progress -- to be discussed}
\begin{enumerate}
    \item CCA limitations: cca with one-hot and cca with glove don't tell us different things. Relative differences between cca scores are not informative (as can be understood by comparing between cca-word and word discriminability)? What does this tell us about the ups and downs in the trends being informative?
    \item Other measures:
    \begin{enumerate}
        \item mutual information is unreliable? Dependence on number of clusters. Can add results on mi-word vs cca-word and mi-phone vs cca-phone.
        \item CKA vs NC vs CCA vs RSA: Differences in trends? Differences in properties measured?
    \end{enumerate}
\end{enumerate}


==> sections/old_versions/efficient-tuning.tex <==
\newpage
\chapter{Towards efficient adaptation of \sfms}
\label{ch:efficient-tuning}
\thispagestyle{plain}
Pre-trained representations from \sfms \ have provided a new standard for solving speech applications~\cite{mohamed2022self}, and a variety of \sfm-specific adaptation strategies have started to emerge~\cite{tsai2022superb, chen2023chapter}. But, despite the wide adoption of \sfms, the community still lacks a standardized adaptation strategy or a principled approach to designing one. Considering the increasing size of \sfms, of the order of 100M to billions~\cite{radford2023robust,borsos2023audiolm,zhang2023google} of parameters, it is unquestionably challenging to design an \sfm-specific strategy for a task without developing some understanding of its intermediate representation space. We seek to leverage insights from our task-agnostic layer-wise analysis (\sect~\ref{sec:analysis}) to motivate design decisions for adaptation strategies. 

\ap{unpolished TBA} \cite{chang2023self} see that phone PNMI and layer-wise probing WER and PER are correlated.

\section{Background}
\input{figures-tex/adapt-strat}
A typical \sfm \ combines a convolutional module followed by self-attention layers. Since the task-specific output label space is typically different from the pre-trained model, a prediction head is added to the \sfm \ before training on the task-specific data. While retaining the convolutional sub-module without fine-tuning is now standard, only a handful of papers studying speaker-related tasks try an alternate approach~\cite{wang2021fine, chen2023chapter}. Additionally, there are multiple possible design options depending on the placement of the prediction head, the input to the prediction head (a single layer or an aggregate of all layers), and the decision to keep the pre-trained parameters frozen or to tune them on the supervised loss. 

Some popular choices are illustrated in \fig~\ref{fig:adapt-strat}. \sfl \ and \afl \ retain the pre-trained \sfm \ parameters as is whereas, \tff \ fine-tunes them on the supervised loss. \afl \ learns a weighted combination of representations from all layers~\cite{tsai2022superb}, whereas \sfl \ uses a single intermediate layer output. 

In this part, we focus on these popular adaptation approaches. Specifically, in \sect~\ref{sec:cca-transfer}, we establish the applicability of our task-agnostic CCA-based analysis for task performance, following which we draw implications for \afl \ and \tff \ in \sects~\ref{sec:adapt-afl} and~\ref{sec:adapt-tff}.

\section{Does CCA measure transferability?}
\label{sec:cca-transfer}
\input{tables-tex/corr-scores}
\input{figures-tex/corr-scores}

We establish that task-agnostic CCA scores (from \sect~\ref{sec:analysis}) reasonably measure a layer's transferability to downstream tasks. We ask whether an \sfm \ layer that is rich in a specific property is also better suited for a downstream task when that task could benefit from the knowledge of that property. To that end, we study the relationship between layer-wise phone/word content and the layer-wise \sfl \ performance on downstream tasks. We choose two tasks related to {\it token-level recognition} --- automatic speech recognition (ASR) and phone recognition (PR) --- and two tasks related to {\it semantic content} --- intent classification (IC) on fluent speech commands and scenario classification on SLURP dataset~\cite{Bastianelli2020SLURPAS}. 
% The first three tasks are from the SUPERB package~\cite{yang2021superb}. 
The relationship is measured as a correlation between layer-wise CCA scores and layer-wise task performance (\tab~\ref{tab:corr-scores}). We measure Spearman’s $\rho$ rank correlation to account for potentially non-linear relationships. 

Semantic task (SLURP and IC) performance is much more correlated with \ccaword \ than with \ccaphone \ (\ccaphone \ is not shown here), which is expected as these semantic tasks should benefit more from word information than phone information. PR and ASR performance are well-correlated with both \ccaphone \ and \ccaword \ scores, except \wavtovec-\baseM \ on ASR. \fig~\ref{fig:scatter} shows scatter plots for four of the settings from \tab~\ref{tab:corr-scores}, including this low-scoring correlation setting. We note that most top-performing layers also have a high CCA score, even though Spearman's correlation does not capture this well in the presence of some outliers. Thus, we establish that representations from layers with high CCA scores also succeed at transferring the encoded property to the downstream task. 

\subsection{CCA for comparative \sfm \ ranking}
Next, we investigate whether CCA scores are comparable across models. For instance, two layers from different \sfms \ with the same CCA score could have different \sfl \ scores. In order to quantify the across-model comparison, we compute the correlation between scores from multiple \sfms \ that are combined based on either the size or the pre-training objective. These are listed in the last four rows of \tab~\ref{tab:corr-scores}. Correlation scores are consistently high except SLURP and ASR when evaluated on \wavtovec. This suggests that comparing CCA scores across models is possible, although with some caveats. We leave further exploration of these caveats to future work (discussed in the proposed work \sect~\ref{sec:proposed}). 

\section{Implications for \afl}
\label{sec:adapt-afl}
\input{figures-tex/weighted-layer-scores}

As our analysis established the varying utility of different layers, we question the use of all layers in \afl. To answer this, we compare the results from \afl \ with the best \sfl \ score (y-axis of \fig~\ref{fig:scatter}). \fig~\ref{fig:task-scores} shows the scores from \afl \ and the best \sfl \ performance, along with the best layer for the latter. We not only find that the best \sfl \ performance is at least as good as \afl \ performance for most tasks but also that the best-performing layer is always lower than at least the top two layers and is close to the layers observed to have the most phonetic and word-level content as measured by CCA (see \figs~\ref{fig:res-cca-phone} and~\ref{fig:res-cca-word}). Specifically, for all semantic tasks, the best-performing layer is one of the top 3 in terms of \ccaword, and for ASR and PR, the best-performing layer is one of the top 6 in terms of both \ccaphone \ and \ccaword. Thus, our CCA-based analysis framework can effectively help narrow down the choice of layers relevant to a downstream task, thus reducing the compute requirements for downstream task adaptation compared to using all layers in \afl.

% We acknowledge that although analyses like ours often indicate downstream performance, task performance also depends on the modeling and optimization issues. For example, layers 22 and 24 of \wavtovec-\largeM \ do not converge on ASR despite having a non-trivial \ccaphone \ score of 0.6; layers 11 and 12 of \wavtovec-\baseM \ have a decent recognition score despite having lower CCA scores than almost all layers (see \fig~\ref{fig:scatter}).

Alternatively, to the presented approach, it is natural to ask whether the layer weights learned in \afl \ experiments are a good indicator of usefulness for downstream tasks. The learned layer weights in \afl \ strategy and the \sfl \ performance have a mean rank correlation of 0.66 across all ten (task, model) pairs. In contrast, the mean rank correlation between \ccaword  \ and task performance is 0.90, even though \ccaword \ is a generic measure while layer weights are task-specific. This further strengthens our proposed analysis-driven design, much lighter than training an \afl \ model to obtain layer importances.

% The relative unreliability of layer weights as an analysis tool is not too surprising and is similar to findings for attention weights in NLP models~\cite{jain2019attention, wiegreffe2019attention}.

\section{Implications for \tff}
\label{sec:adapt-tff}
\input{figures-tex/res-cca-inter}
We know from our previous analysis that the linguistic content that should be helpful for ASR is less well represented in the final few layers of \wavtovec \ (\ccaphone \ in \fig~\ref{fig:res-cca-phone} and \ccaword \ in \fig~\ref{fig:res-cca-word}). We also study the effect of \tff \ on \wavtovec-\baseM \ by computing the CCA similarity between frame-level representations from the corresponding layers of the pre-trained and fine-tuned models ({\it CCA-inter}).\footnote{ASR fine-tuned \wavtovec-\baseM \ is obtained from the fairseq public repo.} As expected, we see that the last few layers of \wavtovec-\baseM \ change the most during \tff \ (\fig~\ref{fig:res-cca-inter}). Based on these observations, we hypothesize that some final layers do not provide a good initialization for the task. To test this hypothesis, we modify the standard \tff \ approach by re-initializing the top layer(s) before performing \tff. We find that re-initializing the final 1-3 layers indeed outperforms the standard approach of initializing all layers from the pre-trained \sfm \ (\tab~\ref{tab:w2v2-asr}), with significant improvements when fine-tuning on the 10-minute training set and minor improvements for larger training sets.

\input{tables-tex/w2v2-asr}

\section{Summary}
In this chapter, we draw on the analytical insights from our task-agnostic CCA-based study (\sect~\ref{sec:analysis}) to derive implications for task-specific adaptation of \sfms. We develop some understanding of how the most popular adaptation strategies, \afl \ and \tff, interact with \sfms, and we consequently suggest modifications that lead to either more efficient or better-performing task-specific models. Specifically, in our study of \afl \ approaches, which have been widely adopted since their introduction~\cite{tsai2022superb}, our study of a few fundamental acoustic-linguistic properties leads to meaningful implications for various tasks. Our approach is more scalable than popular task-specific probing approaches for layer-wise analysis~\cite{shah2021all, feng2022silence, ji2022predicting}, and our analysis techniques are easily extensible to additional properties besides the ones we have studied here (e.g., speaker, prosody, syntax). 

==> sections/old_versions/intro_old.tex <==
% \newpage
\section{Introduction}
\label{sec:intro}

For the past several decades, the majority of speech technologies have used some form of spectrogram features to pre-process dense raw speech signals into compact, low-resolution representation vectors~\cite{flanagan2013speech}.
The discovery of speech spectrogram features, motivated by human perception of speech, has been one of the biggest breakthroughs in speech research~\cite{tbd}\tbd{what will be a good reference to add here? I am looking for maybe the first time spectrogram features were proposed, maybe Sadaoki's dynamic features paper?}.
The majority of speech tasks since have used some variant of spectrogram features as a way to pre-process the dense raw speech signals to extract compact, low-resolution representation vectors.

\tbd{Introduce self-supervised speech representations}
It is remarkable that self-supervised speech representations, trained on large amounts of unlabeled audio, have almost ubiquitously replaced these spectrogram features within the last four years~\cite{mohamed2022self, borgholt2022brief}.
In fact, the most recent speech representation models~\cite{hsu2021hubert, chen2022wavlm} seem to be learning general representations that are useful for diverse tasks that rely on very different types of information -- phonetics, speaker, spoken content, paralinguistics~\cite{yang2021superb}. However, these models are huge (of the order of 100M parameters), computationally demanding, and not well understood\tbd{"not well understood" is vague}. \tbd{Add a connector sentence. What problem/challenge is the first part of my work solving?}
{\it In the first part of my work, I adopt lightweight analysis tools to understand these models\tbd{"understand these models" is vague}. We measure the acoustic-linguistic properties encoded in the self-supervised representations across layers}~\cite{pasad2021layer, pasad2022comparative} {\it and going further, I plan to analyse the semantic content and contextualization in these models}.

% {\it In the first part of my work, I seek to answer: What makes these representation models, trained on raw audios, successful? I adopt lightweight analysis tools to develop an understanding of the representation structure and properties induced by self-supervised training}~\cite{pasad2021layer, arxiv}.

Adaptation of self-supervised speech models for downstream tasks, referred as fine-tuning, is both effective and data-efficient~\cite{mohamed2022self, yang2021superb, shon2022slue}.
% These are then adapted for downstream tasks, typically using a prediction head on top that is trained with the supervised task loss. This approach, referred to as fine-tuning, is both effective and data efficient
For instance, for automatic speech recognition (ASR) it is now common to benchmark performance using just 10 minutes to 10 hours of labeled training data\tbd{, as opposed to typical 1000s of hours ...}.
However, fine-tuning often comes with huge compute and memory cost, and
% all the model parameters are tuned in the process, so this comes at a huge memory and compute cost. 
% \and unsupervised ASR has become feasible too~\cite{baevski2021unsupervised}.
% It is common to evaluate these models on a diverse set of tasks beyond ASR~\cite{yang2021superb}, but
there is no standardized fine-tuning strategy or a principled approach for designing one. 
{\it In the second part of my work, I study self-supervised models in the context of downstream tasks, and use the insights to propose more effective and/or efficient fine-tuning protocols}~\cite{pasad2021layer, xie2022hidden, pasad2022comparative}. 

The data efficiency benefits of pre-trained models are particularly attractive for spoken language understanding (SLU) since these tasks typically have limited labeled data. Since SLU tasks require contextual understanding beyond just surface form characters and words,
it is not evident that the SLU will enjoy the same benefits as other speech tasks.
% benefits seen for other speech processing tasks will apply to SLU. 
{\it 
% In order to facilitate progress on this subject, 
In order to facilitate more investigation in this direction,
I am one of the developers of the spoken language understanding evaluation (SLUE) benchmark}~\cite{shon2022slue, pasad2021use}{\it. The third part of my proposed work combines insights from SLU tasks and analysis tools to propose improvements to pre-trained models for semantic tasks.}

% Spoken language understanding tasks have mostly been tackled using semi-supervised techniques. 

% The data efficiency benefits of these models also extend to spoken language understanding (SLU) tasks~\cite{shon2022slue}. 

% (ATIS is low resource)
% This is a little surprising since the extent of semantic content in the pre-trained representations is unclear~\cite{pasad2021layer} (as is discussed in Sec.~\ref{sec:study}) and SLU tasks typically require contextual .


% Importance of SLU tasks \\
% These tasks have become especially important since automated speech assistants have become ubiquitous.

% Why is SLU challenging? \\
% When comparing to natural language understanding (text inputs),
% performing inference on speech is even more challenging owing to the dense, continuous and unsegmented
% input.

% This is true for any speech task \\
% Additionally, acoustic and speaker variability add challenges beyond linguistic variability, and this
% could compound data requirements if we were to solely rely on supervised learning techniques.

% Large scale pre-training has made it feasible to consider tasks with limited labeled data.

% SLU datasets are also typically small, thus making it a common practice to rely on alternate source of supervision
% (typically ASR models), either in transfer learning setup [?] or a pipeline setup [?]. Even amongst the
% SLU datasets that we have [add what’s missing]

% In my work, I seek to supplement the unequivocal success stories of the self-supervised models the community has seen so far, with (i) a study of these models to develop an understanding of the representation structure and properties induced by self-supervised training~\cite{pasad2021layer, arxiv}; (ii) an examination of how these findings relate to the existing efforts on downstream tasks, and consequently, effective fine-tuning strategies that our study inspires~\cite{pasad2021layer, emnlp}; and (iii) a natural data spoken language understanding evaluation (SLUE) benchmark, an in-depth study of modeling approaches for SLU leveraging the pre-trained models, and consequently, a pre-training strategy to learn representations that learn semantics, motivated by our study of existing representations and SLU tasks~\cite{shon2022slue, pasad2021use}.    

% \begin{enumerate}
%     \item What do the pre-trained representations encode? \\
%     We seek to complement the empirical evidence with a non-parametric analysis of representations learned in a self-supervised fashion. How do we even measure semantic content in self-supervised tasks? Additionally, we also look at how fine-tuning changes these trends, and seek to find any efficient fine-tuning strategies. 
%     \item Implications for downstream tasks \\
%     We extend the findings and analysis tools from above to derive observations and practical strategies for developing effective performance on downstream tasks.
%     \item Spoken language understanding \\
%     We specifically focus on a realistic setting of limited labeled SLU. We describe ongoing work on creating a benchmark and share our findings. 
    
% \end{enumerate}






==> sections/old_versions/proposed.tex <==
\newpage
\chapter{Proposed work}
\label{sec:proposed}
% \thispagestyle{plain}
% chatgpt done

We aim to contribute to our ongoing efforts to understand the evolving landscape of \sfms. We plan to expand our investigation to encompass new \sfms \ and improved adaptation strategies. Additionally, we intend to conduct a comprehensive study comparing popular lightweight analysis tools with our CCA-based analysis framework.

\section{Study of (weakly) supervised \sfms}
In \sect~\ref{sec:analysis}, we analyze several \sfms \ varying in their pre-training objective (contrastive as well as predictive objectives), input modality (visually grounded as well as speech-only models), pre-training data (both in terms of size and language), and the size of the model. In \sect~\ref{sec:slu}, we used some of these \sfms \ as a backbone for solving complex language understanding tasks. 

More recently, weakly supervised speech recognition models such as Whisper~\cite{radford2023robust} and USM~\cite{zhang2023google} are starting to become a competitive choice as a backbone for language understanding tasks~\cite{gong2023joint, le2023voicebox, cheng2023mu}. These models are larger by order of magnitude in terms of the number of parameters and the amount of pre-training data. We plan to extend our analysis to these supervised \sfms \ and also benchmark their capabilities for language understanding tasks from our SLUE benchmark. Some of the recent work has shown that speech-only \sfms \ fine-tuned for speech recognition might offer a better backbone for SLU tasks~\cite{arora2022espnet, shon2023slue, peng2023study}, so these weakly supervised \sfms \ may be better suited for SLU tasks than speech-only \sfms.

Considering the difference in scale and the pre-training task, we expect to see differences in the properties encoded by these models, just like how visually grounded \sfms \ have different strengths in comparison to speech-only \sfms \ and how \largeM \ models vary in their layer-wise trends when compared to their \baseM \ counterparts. 

\section{Comparative study of analysis tools}
Our current analysis, outlined in \sect~\ref{sec:analysis}, relies on canonical correlation analysis and some unsupervised tasks. In our study, projection-weighted CCA~\cite{morcos2018insights} has proven to be a robust tool, corroborating the findings from task performance trends (\sect~\ref{sec:efficient-tuning}). It has also been a common choice of analysis method in related studies on neural network representations~\cite{morcos2018insights, voita2019bottom}. 

Several other popular tools exist for studying neural network representations. These include variants of CCA~\cite{raghu2017svcca}, neural collapse (NC) ~\cite{papyan2020prevalence}, center kernel alignment (CKA)~\cite{cristianini2001kernel, cortes2012algorithms}, orthogonal Procrustes (OP)~\cite{schonemann1966generalized}, representation similarity analysis (RSA)~\cite{kriegeskorte2008representational}, and discrete mutual information. While some previous studies have discussed the merits and drawbacks~\cite{ding2021grounding, kornblith2019similarity} of some of these methods, these are primarily focused on the similarity analysis between neural network representations. 

Although CCA is lightweight, it involves training and tuning for parameters and hyper-parameters, respectively, and is thus best solved using a cross-validation set-up. In contrast, other metrics like NC, CKA, and RSA are non-parametric and likely faster to compute but might have limitations, such as the need for meticulous data curation for RSA or discrete label constraints for NC. In prior work, we used discrete MI to compare \sfm \ representations with discrete labels~\cite{pasad2021layer}, but we dropped the metric due to its non-interpretable dependence on the clustering step. In another prior work studying text foundation models on classification tasks, we observed correlations between NC and CCA trends~\cite{xie2022hidden}. 

Building upon this groundwork, we aim to investigate these analysis tools' applicability in studying \sfms. In the process, we also hope to find tools particularly suitable for comparing \sfms, expanding further on our preliminary study in \sect~\ref{sec:cca-transfer}. Specifically, a favorable tool should (i) provide a reliable way to measure knowledge encoded across different layers of an \sfm \ and (ii) generate scores that offer a reliable ranking of \sfms.
% Specifically, these tools should offer quantitative metrics comparable across various models and, thus, provide more comprehensive insights beyond individual \sfms' layer-wise trends.
We will release a suite of the most effective tools for the ease of reusability.

\section{Implications for parameter-efficient tuning}
% \thispagestyle{fancy}
% \fancyhead[L]{Proposed work}  % Change as needed
% \fancyhead[R]{}  % Change as needed

Various strategies exist to adapt an \sfm \ (\fig~\ref{fig:adapt-strat}). While \tff \ typically outperforms frozen layer methods (\sfl \ or \afl), its computational demands escalate as \sfms \ grow in size. Full-finetuning approaches, such as \tff, are not space efficient either, as each task-specific tuning creates a different model with the same size as the backbone \sfm. 

More recently, parameter-efficient tuning (PET) approaches, initially developed for text foundation models~\cite{he2021towards, houlsby2019parameter}, have gained traction in the context of \sfms~\cite{chen2023exploring, chang2023prompting, li2023evaluating}. These task-specific models leverage the pre-trained \sfm's frozen parameters and utilize a significantly smaller set of additional parameters, in contrast to the \sfm's overall size. Thus, PET approaches eliminate the need to fine-tune all \sfm \ parameters and introduce only a manageable overhead of task-specific parameters. We aim to employ our analytical tools to understand how these adaptation techniques interact with the pre-trained representations. Consequently, we hope to derive guidance on best positioning these parameter-efficient modules within an \sfm, further reducing the parameter size of PET algorithms.

Previous studies~\cite{thomas2022efficient, huang2023findadaptnet} have explored different placements of adapter modules~\cite{houlsby2019parameter} and have compared it to the conventional practice of adding a module at each layer. But these studies either use heuristic measures such as using {\it top-k} layers~\cite{thomas2022efficient} or require training a task-specific \afl \ model~\cite{huang2023findadaptnet}. In a related prior work with NLP collaborators~\cite{xie2022hidden}, we use neural collapse~\cite{papyan2020prevalence} to measure the task specificity of different layers of pre-trained text representation models and consequently decide whether to freeze/fine-tune or retain/drop particular layers. This process results in efficient fine-tuning approaches that are comparable to \tff \ strategy. In the same work, we also establish the applicability of CCA for this purpose. We expect to find similar principled strategies for adapting \sfms \ using PET approaches.




==> sections/old_versions/timeline.tex <==
\newpage
\chapter{Timeline}
% \thispagestyle{plain}

\paragraph{Study of supervised \sfms}    January 2024-March 2024 
\begin{itemize}
	\item Layerwise analysis of acoustic and linguistic properties for Whisper~\cite{radford2023robust} and OWSM~\cite{peng2023reproducing} models.
	\item Provide Whisper and OWSM-based baselines for SLU tasks, specifically named entity recognition and localization. Use adaptation strategies including but not limited to \sfl \ and \afl.
\end{itemize}


 \paragraph{Comparative study of analysis tools} March 2024-April 2024
\begin{itemize}
 \item Use alternate analysis tools to perform layerwise studies for a subset of \sfms \ and compare the trends with our previous CCA-based analysis. 
 \item Develop an intuition for how the various tools differ and whether certain tools may be preferable for \sfm \ analysis than others.
\end{itemize}

\paragraph{Study of parameter efficient tuning (PET) techniques} April 2024-June 2024
\begin{itemize}
 \item Study how the parameter efficient tuning strategies change the intermediate \sfm \ representations and use the analytical insights to place PET modules within the \sfm \ layers.
\end{itemize}

\paragraph{Job Search} May 2024-July 2024

\paragraph{Thesis Writing} May 2024-August 2024

\paragraph{Thesis Defense} August 2024

==> sections/related-work-our-work.tex <==
\noindent {\bf Where does our work fit in?}\\
\ap{yet to figure out where to place this}
Analysis of higher-level units, such as words in S3Ms, has been limited. 
Pasad et al.\cite{pasad2023comparative} analyzed the extent to which different layers of S3Ms encode word identity, and Sanabria et al.\cite{sanabria2023analyzing} found that pooled S3M representations over word segments perform competitively on the task of acoustic word discrimination.  These results indicate that S3Ms encode word-identifying information.  However, it is not clear from prior work how word information is distributed across frames and what aspects of words are encoded, such as their pronunciation, syntactic properties, or semantic properties; our work addresses this gap.

Task-specific probing classifiers have been a common analysis tool for speech models~\cite{belinkov2019analysis,palaskar2019learned,prasad2020accents} including S3Ms~\cite{hsu2021hubert,baevski2021unsupervised,ma2021probing,shah2021all,shen2023wave}. While these probes provide an intuitive evaluation measure, 
the design decisions involved in training task-specific classifiers have confounding effects, making the scores hard to interpret~\cite{hewitt2019designing, ravichander2020probing, belinkov2022probing}. We use canonical correlation analysis (CCA)~\cite{harold1936relations} and training-free task-based evaluation, thus bypassing the dependence on task-specific classifiers. 

CCA and its more robust variants have been previously used to compare representations within and across neural networks~\cite{raghu2017svcca, kornblith2019similarity}, to study text representation models~\cite{voita2019bottom,tsvetkov2016correlation,saphra2019understanding}, and more recently for the analysis of S3M representations~\cite{pasad2021layer, li2023exploration, pasad2023comparative, yang2023can}. While classifiers require discrete labels, CCA can be used with both discrete and continuous-valued labels. CCA is also computationally inexpensive and has a closed-form solution.

Word similarity (WordSim) tasks~\cite{faruqui2014community} have been commonly used for intrinsic evaluation of word vectors. However, previous work has observed some problematic aspects of these tasks~\cite{faruqui2016problems}, including that WordSim performance is not well-correlated with extrinsic evaluation, whereas CCA-based evaluation more consistently tracks downstream task performance~\cite{tsvetkov2016correlation}.
Our work also shares some motivation with the Zero Resource Speech Benchmark~\cite{nguyen2020zero}, but tasks in this benchmark require encoding isolated word segments and/or discretizing the representations. Our analyses use word segment representations extracted in context, in order to match the most common use cases of S3Ms.

The task of acoustic word discrimination (AWD)~\cite{carlin2011rapid} has been commonly used to evaluate segment-level acoustic word embeddings, using both unsupervised~\cite{levin2013fixed,peng2020correspondence,algayres2020evaluating,van2021comparison} and supervised models~\cite{kamper2016cnn_awe,settle2016discriminative,he2017multiview,algayres2020evaluating}.  To our knowledge, only Sanabria et al.\cite{sanabria2023analyzing} and Van et al.\cite{van2021comparison} have studied the use of S3Ms for generating acoustic word embeddings for AWD.  Van et al.\cite{van2021comparison} used "first-generation" S3Ms while~\cite{sanabria2023analyzing} analyzed two of the same modern S3Ms we study here.  Our work provides a more comprehensive study of using multiple approaches (unsupervised mean pooling, dynamic time warping, and supervised models using S3M features), as well as a new state-of-the-art for one of the most commonly used AWD benchmarks.

Word unit discovery and segmentation are common benchmark tasks that have also been used to study speech representations~\cite{dunbar2020zero, nguyen2022word, sanabria2021difficulty, algayres2022dp, bhati2021segmental, cuervo2022contrastive, ten2007computational}.
Previous work studying the segmentation capabilities of S3Ms includes~\cite{kamper2022word}, based on first discovering phone-like units and then using them to discover word segments, and~\cite{peng2022word}, based on thresholding the attention map of a visually grounded speech model (VG-HuBERT, which we also use here).  Our study complements this prior work by comparing the layer-wise performance of a large number of S3Ms for this task and showing that a simple, training-free segmentation algorithm performs very competitively.

Textual sentence similarity is a classic task in NLP~\cite{conneau2018senteval}, but there are only a few studies investigating {\it spoken} utterance representations for this task~\cite{merkx2021semantic, merkx2023modelling, zhu2022bootstrapping}. Some downstream tasks in the SUPERB benchmark~\cite{yang2021superb} successfully use spoken utterance representations from frozen S3Ms, represented by a single mean-pooled vector. We complement our understanding of the capabilities of pooled utterance representations by performing a broad cross-model comparison.

==> tables-tex/corr-scores.tex <==

\begin{table}[t]
\centering
\footnotesize
\caption{Spearman's $\rho$ correlation scores between layer-wise CCA scores and \sfl \ task performance. Lighter the color of the cell, better the correlation score, and a higher correlation implies better transferability.}
\begin{tabular}{ll|llllll}
\hlineB{2}
% \rowcolor{gray!50} % header row color
% \rowcolor[RGB]{230,230,230}
\multicolumn{2}{l}{Downstream task} & \multicolumn{2}{|c}{PR} & \multicolumn{2}{c}{ASR} & \multicolumn{1}{c}{SLURP} & \multicolumn{1}{c}{IC} \\
\multicolumn{2}{l}{Layer-wise trend} & \multicolumn{1}{|l}{CCA-phone} & CCA-word & CCA-phone & CCA-word & CCA-word & CCA-word \\
% \rowcolor[RGB]{230,230,230}
\hlineB{2}
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Individual\\ models\end{tabular}} & {\scriptsize \wavtovec-\baseM} & \cellgrad{0.79} & \cellgrad{0.90} & \cellgrad{0.56} & \cellgrad{0.66} & \cellgrad{0.98} & \cellgrad{0.99} \\
& {\scriptsize \hubert-\baseM} & \cellgrad{0.92} & \cellgrad{0.90} & \cellgrad{0.92} & \cellgrad{0.90} & \cellgrad{1.00} & \cellgrad{0.99} \\
& {\scriptsize \wavtovec-\largeM} & \cellgrad{0.80} & \cellgrad{0.68} & \cellgrad{0.76} & \cellgrad{0.71} & \cellgrad{0.90} & \cellgrad{0.88} \\
& {\scriptsize \hubert-\largeM} & \cellgrad{0.84} & \cellgrad{0.95} & \cellgrad{0.84} & \cellgrad{0.95} & \cellgrad{0.96} & \cellgrad{0.90} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Combination\\ of multiple\\ models\end{tabular}} & \begin{tabular}[c]{@{}l@{}}{\scriptsize \wavtovec-\baseM} \ {\scriptsize \&} \\ {\scriptsize \wavtovec-\largeM} \end{tabular} & \cellgrad{0.76} & \cellgrad{0.81} & \cellgrad{0.56} & \cellgrad{0.71} & \cellgrad{0.78} & \cellgrad{0.81} \\ \cline{2-8}
& \begin{tabular}[c]{@{}l@{}}{\scriptsize \hubert-\baseM} \ {\scriptsize \&} \\ {\scriptsize \hubert-\largeM} \end{tabular} & \cellgrad{0.85} & \cellgrad{0.92} & \cellgrad{0.83} & \cellgrad{0.93} & \cellgrad{0.97} & \cellgrad{0.94} \\ \cline{2-8}
& \begin{tabular}[c]{@{}l@{}} {\scriptsize \wavtovec-\baseM} \ {\scriptsize \&} \\ {\scriptsize \hubert-\baseM} \end{tabular} & \cellgrad{0.86} & \cellgrad{0.92} & \cellgrad{0.73} & \cellgrad{0.79} & \cellgrad{0.93} & \cellgrad{0.95} \\ \cline{2-8}
& \begin{tabular}[c]{@{}l@{}} {\scriptsize \wavtovec-\largeM} \ {\scriptsize \&} \\ {\scriptsize \hubert-\largeM} \end{tabular} & \cellgrad{0.83} & \cellgrad{0.87} & \cellgrad{0.77} & \cellgrad{0.87} & \cellgrad{0.93} & \cellgrad{0.92}
\end{tabular}

\label{tab:corr-scores}
\end{table}

==> tables-tex/segmentation.tex <==
\begin{table}[tbh]
  \begin{minipage}[c]{0.7\textwidth}
    \setlength{\tabcolsep}{4pt}
    \small
    \centering
    \begin{tabular}{l r r r r}
        \toprule
        Method & Prec. & Rec. & F-1 & R-val. \\
        \midrule
        \textit{Prior work\protect\footnotemark} \\
        \hspace{2mm} DPDP~\cite{kamper2022word}  & 35.3 & 37.7 & 36.4 & 44.3 \\
        \hspace{2mm} \vghubert~\cite{peng2022word} & \multirow{1}{*}{\bf{36.2}} & \multirow{1}{*}{32.2} & \multirow{1}{*}{34.1} & \multirow{1}{*}{\bf{45.6}} \\
        \midrule
        \multicolumn{5}{l}{\textit{Ours (Best Layer)}} \\
        \hspace{2mm} \wavlm-\baseM \ (L8) &  31.9 & 45.7 & 37.6 &30.7\\ 
        \hspace{2mm} \hubert-\baseM \ (L9) & 33.8 &  46.6 & 39.2 & 34.9 \\ 
        \hspace{2mm} \wavtovec-\baseM \ (L7) & 27.0 & 47.2 & 34.3 & 8.9\\ 
        \hspace{2mm} \vghubert \ (L10) & 36.0 & \bf{47.6} & \bf{41.0} & 39.5\\ 
        \bottomrule 
    \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.3\textwidth}
    \caption{Word segmentation performance on Buckeye test set. Higher is better for all metrics.}
  \label{tab:word_seg}
  \end{minipage}
\end{table}


==> tables-tex/vp-stats.tex <==
\begin{table*}[h]
\centering
\small
% \resizebox{1.0\linewidth}{!}{%
\begin{tabular}{l|rrr|l|l|l}
\hlineB{2}
\multirow{2}{*}{Corpus} & \multicolumn{3}{c|}{Size - utts (hour)}  & \multirow{2}{*}{Speech type} & \multirow{2}{*}{Source domain} & \multirow{2}{*}{License} \\ \cline{2-4}
 & \multicolumn{1}{c}{Fine-tune} & \multicolumn{1}{c}{Dev} & \multicolumn{1}{c|}{Test} &  & &\\ \hlineB{2}
SLUE-VoxPopuli  & 5,000 (14.5)  & 1,753 (5.0)  & 1,842 (4.9) & Scripted & European parliament & CC0\\ \hline
\end{tabular}%
% }
\caption{Corpus statistics and task descriptions. 
}
\label{tab:vp-stats}
\end{table*}



% \begin{table*}[h]
% \centering
% \resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l|r|rrr|l|l|l|l}
% \hlineB{2}
% \multirow{3}{*}{Corpus} & \multicolumn{4}{c|}{Size - utts (hour)} & \multirow{3}{*}{Tasks} & \multirow{3}{*}{Speech type} & \multirow{3}{*}{Source domain} & \multirow{3}{*}{License} \\ \cline{2-5}
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unlabeled\\(in-domain)\end{tabular}} & \multicolumn{3}{c|}{Labeled} & & &\\ \cline{3-5}
%  & & \multicolumn{1}{c}{Fine-tune} & \multicolumn{1}{c}{Dev} & \multicolumn{1}{c|}{Test} &  & & &\\ \hlineB{2}
% SLUE-VoxPopuli & 195,655 (5,122)  & 5,000 (14.5)  & 1,753 (5.0)  & 1,842 (4.9) & ASR, NER & Scripted & European parliament & CC0\\ \hline
% SLUE-VoxCeleb & 1.27M (2,780) & 5,777 (12.8) & 955 (2.1) & 4,052 (9.0)  & ASR, SA & Conversational & Broadcasting (YouTube) & CCBY 4.0\\ \hlineB{2}
% % (Librispeech) & - (60,000h) & (10h) & (5h) & (5h) & ASR & Reading written text & eBooks & CC BY 4.0\\ \hlineB{2}
% \end{tabular}%
% }
% \caption{Corpus statistics and task descriptions. \kl{this is better but still a bit small.  could remove the license column and just mention the license in the caption.}
% % \kl{could save space here by removing the "h"s (the column heading mentions that these are hours), replacing "natural conversation" with "conversational" and "scripted speech" with "scripted", and replacing 195,655 with 196M.  BTW does 1.27m mean 1.27 million?  If so I think it should be "M".}
% }
% \label{tab:tasks_description}
% \end{table*}
